Smart City Development with Urban Transfer Learning

Nowadays, the smart city development levels of different cities are still unbalanced. For a large number of cities which just started development, the governments will face a critical cold-start problem: 'how to develop a new smart city service with limited data?'. To address this problem, transfer learning can be leveraged to accelerate the smart city development, which we term the urban transfer learning paradigm. This article investigates the common process of urban transfer learning, aiming to provide city planners and relevant practitioners with guidelines on how to apply this novel learning paradigm. Our guidelines include common transfer strategies to take, general steps to follow, and case studies in public safety, transportation management, etc. We also summarize a few research opportunities and expect this article can attract more researchers to study urban transfer learning.

==> conclusions.tex <==
%!TEX root = transfer_in_smart_city.tex
\section{Conclusions}

This article gives a systematic view of urban transfer learning to address cold-start problems in smart city development. We analyze the common strategies and general process framework for urban transfer learning applications. We expect that this article can attract more research efforts into this research area.


